Pattern Analogies: Learning to Perform Programmatic Image Edits by Analogy

Pattern images are everywhere in the digital and physical worlds, and tools to edit them are valuable. But editing pattern images is tricky: desired edits are often programmatic: structure-aware edits that alter the underlying program which generates the pattern. One could attempt to infer this underlying program, but current methods for doing so struggle with complex images and produce unorganized programs that make editing tedious. In this work, we introduce a novel approach to perform programmatic edits on pattern images. By using a pattern analogy -- a pair of simple patterns to demonstrate the intended edit -- and a learning-based generative model to execute these edits, our method allows users to intuitively edit patterns. To enable this paradigm, we introduce SplitWeave, a domain-specific language that, combined with a framework for sampling synthetic pattern analogies, enables the creation of a large, high-quality synthetic training dataset. We also present TriFuser, a Latent Diffusion Model (LDM) designed to overcome critical issues that arise when naively deploying LDMs to this task. Extensive experiments on real-world, artist-sourced patterns reveals that our method faithfully performs the demonstrated edit while also generalizing to related pattern styles beyond its training distribution.

==> figures/banner.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=1.00\linewidth]{resources/banner.png}
	\caption{We introduce a system for making \textit{programmatic} edits on pattern images without inferring their underlying programs. 
 }
\label{fig:teaser}
\end{figure}

==> figures/datagen_eval.tex <==
% Should be a plot on program distance A, B vs Loss.
\begin{figure}[t!]
	\centering
 % \includegraphics[width=.32\linewidth]{example-image-a.png}
	\includegraphics[width=0.70\linewidth]{example-image-a.png}
	\caption{ graph showing program distance vs prompt fidelity metric
 }
\label{fig:teaser}
\end{figure}

==> figures/feature_encoding.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=1.00\linewidth]{resources/image_encoding.png}
	\caption{ 
 }
\label{fig:teaser}
\end{figure}

==> figures/splitweave_prog.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=1.00\linewidth]{resources/splitweave_program.png}
	\caption{ 
 }
\label{fig:teaser}
\end{figure*}

==> figures/wider_canvas.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=1.00\linewidth]{resources/wider_canvas.png}
	\caption{ 
 }
\label{fig:teaser}
\end{figure}

==> latexmkrc.tex <==
#!/usr/bin/perl

## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.15;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";

==> tables/ablation.tex <==

\setlength{\tabcolsep}{2pt}
\newdimen\wate \wate=30pt
\newdimen\wperc \wperc=24pt

\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@1} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.624} & \cellCD[\wate]{e0a4a4}{0.821} & \cellCD[\wate]{e0a4a4}{0.422} & \cellCD[\wate]{e0a4a4}{0.479} \\
no\_type & \cellCD[\wate]{e3e6bd}{0.270} & \cellCD[\wate]{e3e6bd}{0.498} & \cellCD[\wate]{fdf0cf}{0.560} & \cellCD[\wate]{f6f0cb}{0.308} \\
no\_lower & \cellCD[\wate]{a8c992}{0.124} & \cellCD[\wate]{a8c992}{0.380} & \cellCD[\wate]{cfdcae}{0.617} & \cellCD[\wate]{a8c992}{0.223} \\
no\_dino & \cellCD[\wate]{a8c992}{0.146} & \cellCD[\wate]{bbd2a0}{0.417} & \cellCD[\wate]{cfdcae}{0.623} & \cellCD[\wate]{bbd2a0}{0.245} \\
ours & \cellCD[\wate]{a8c992}{0.118} & \cellCD[\wate]{a8c992}{0.365} & \cellCD[\wate]{a8c992}{0.644} & \cellCD[\wate]{a8c992}{0.215} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@2} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.609} & \cellCD[\wate]{e0a4a4}{0.811} & \cellCD[\wate]{e0a4a4}{0.439} & \cellCD[\wate]{e0a4a4}{0.466} \\
no\_type & \cellCD[\wate]{e3e6bd}{0.214} & \cellCD[\wate]{e3e6bd}{0.450} & \cellCD[\wate]{fdf0cf}{0.598} & \cellCD[\wate]{e3e6bd}{0.277} \\
no\_lower & \cellCD[\wate]{a8c992}{0.103} & \cellCD[\wate]{a8c992}{0.355} & \cellCD[\wate]{e3e6bd}{0.634} & \cellCD[\wate]{a8c992}{0.207} \\
no\_dino & \cellCD[\wate]{a8c992}{0.124} & \cellCD[\wate]{bbd2a0}{0.380} & \cellCD[\wate]{cfdcae}{0.646} & \cellCD[\wate]{bbd2a0}{0.231} \\
ours & \cellCD[\wate]{a8c992}{0.090} & \cellCD[\wate]{a8c992}{0.327} & \cellCD[\wate]{a8c992}{0.671} & \cellCD[\wate]{a8c992}{0.199} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@4} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.591} & \cellCD[\wate]{e0a4a4}{0.796} & \cellCD[\wate]{e0a4a4}{0.447} & \cellCD[\wate]{e0a4a4}{0.457} \\
no\_type & \cellCD[\wate]{cfdcae}{0.174} & \cellCD[\wate]{cfdcae}{0.405} & \cellCD[\wate]{e3e6bd}{0.636} & \cellCD[\wate]{e3e6bd}{0.250} \\
no\_lower & \cellCD[\wate]{a8c992}{0.089} & \cellCD[\wate]{a8c992}{0.339} & \cellCD[\wate]{e3e6bd}{0.650} & \cellCD[\wate]{a8c992}{0.197} \\
no\_dino & \cellCD[\wate]{a8c992}{0.101} & \cellCD[\wate]{a8c992}{0.343} & \cellCD[\wate]{bbd2a0}{0.675} & \cellCD[\wate]{bbd2a0}{0.211} \\
ours & \cellCD[\wate]{a8c992}{0.078} & \cellCD[\wate]{a8c992}{0.308} & \cellCD[\wate]{a8c992}{0.690} & \cellCD[\wate]{a8c992}{0.187} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@5} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.588} & \cellCD[\wate]{e0a4a4}{0.795} & \cellCD[\wate]{e0a4a4}{0.449} & \cellCD[\wate]{e0a4a4}{0.455} \\
no\_type & \cellCD[\wate]{cfdcae}{0.162} & \cellCD[\wate]{cfdcae}{0.388} & \cellCD[\wate]{e3e6bd}{0.646} & \cellCD[\wate]{cfdcae}{0.244} \\
no\_lower & \cellCD[\wate]{a8c992}{0.085} & \cellCD[\wate]{a8c992}{0.334} & \cellCD[\wate]{e3e6bd}{0.653} & \cellCD[\wate]{a8c992}{0.195} \\
no\_dino & \cellCD[\wate]{a8c992}{0.098} & \cellCD[\wate]{a8c992}{0.338} & \cellCD[\wate]{bbd2a0}{0.679} & \cellCD[\wate]{bbd2a0}{0.208} \\
ours & \cellCD[\wate]{a8c992}{0.076} & \cellCD[\wate]{a8c992}{0.305} & \cellCD[\wate]{a8c992}{0.692} & \cellCD[\wate]{a8c992}{0.185} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@8} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.579} & \cellCD[\wate]{e0a4a4}{0.787} & \cellCD[\wate]{e0a4a4}{0.456} & \cellCD[\wate]{e0a4a4}{0.452} \\
no\_type & \cellCD[\wate]{bbd2a0}{0.139} & \cellCD[\wate]{bbd2a0}{0.369} & \cellCD[\wate]{e3e6bd}{0.662} & \cellCD[\wate]{cfdcae}{0.228} \\
no\_lower & \cellCD[\wate]{a8c992}{0.079} & \cellCD[\wate]{a8c992}{0.324} & \cellCD[\wate]{e3e6bd}{0.662} & \cellCD[\wate]{a8c992}{0.189} \\
no\_dino & \cellCD[\wate]{a8c992}{0.091} & \cellCD[\wate]{a8c992}{0.326} & \cellCD[\wate]{bbd2a0}{0.688} & \cellCD[\wate]{bbd2a0}{0.201} \\
ours & \cellCD[\wate]{a8c992}{0.072} & \cellCD[\wate]{a8c992}{0.295} & \cellCD[\wate]{a8c992}{0.704} & \cellCD[\wate]{a8c992}{0.178} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@10} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.578} & \cellCD[\wate]{e0a4a4}{0.784} & \cellCD[\wate]{e0a4a4}{0.459} & \cellCD[\wate]{e0a4a4}{0.451} \\
no\_type & \cellCD[\wate]{bbd2a0}{0.131} & \cellCD[\wate]{bbd2a0}{0.363} & \cellCD[\wate]{e3e6bd}{0.666} & \cellCD[\wate]{cfdcae}{0.225} \\
no\_lower & \cellCD[\wate]{a8c992}{0.078} & \cellCD[\wate]{a8c992}{0.321} & \cellCD[\wate]{e3e6bd}{0.666} & \cellCD[\wate]{a8c992}{0.186} \\
no\_dino & \cellCD[\wate]{a8c992}{0.089} & \cellCD[\wate]{a8c992}{0.322} & \cellCD[\wate]{bbd2a0}{0.691} & \cellCD[\wate]{bbd2a0}{0.199} \\
ours & \cellCD[\wate]{a8c992}{0.070} & \cellCD[\wate]{a8c992}{0.292} & \cellCD[\wate]{a8c992}{0.706} & \cellCD[\wate]{a8c992}{0.177} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@16} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & \cellCD[\wate]{e0a4a4}{0.572} & \cellCD[\wate]{e0a4a4}{0.780} & \cellCD[\wate]{e0a4a4}{0.463} & \cellCD[\wate]{e0a4a4}{0.447} \\
no\_type & \cellCD[\wate]{bbd2a0}{0.120} & \cellCD[\wate]{bbd2a0}{0.350} & \cellCD[\wate]{cfdcae}{0.678} & \cellCD[\wate]{cfdcae}{0.216} \\
no\_lower & \cellCD[\wate]{a8c992}{0.072} & \cellCD[\wate]{a8c992}{0.311} & \cellCD[\wate]{e3e6bd}{0.673} & \cellCD[\wate]{a8c992}{0.180} \\
no\_dino & \cellCD[\wate]{a8c992}{0.084} & \cellCD[\wate]{a8c992}{0.315} & \cellCD[\wate]{bbd2a0}{0.697} & \cellCD[\wate]{bbd2a0}{0.194} \\
ours & \cellCD[\wate]{a8c992}{0.064} & \cellCD[\wate]{a8c992}{0.284} & \cellCD[\wate]{a8c992}{0.713} & \cellCD[\wate]{a8c992}{0.172} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\setlength{\tabcolsep}{2pt}
\newdimen\wate \wate=30pt
\newdimen\wperc \wperc=24pt

\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@1} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.624} & {0.821} & {0.422} & {0.479} \\
no\_type & {0.270} & {0.498} & {0.560} & {0.308} \\
no\_lower & {0.124} & {0.380} & {0.617} & {0.223} \\
no\_dino & {0.146} & {0.417} & {0.623} & {0.245} \\
ours & \textbf{0.118} & \textbf{0.365} & \textbf{0.644} & \textbf{0.215} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@2} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.609} & {0.811} & {0.439} & {0.466} \\
no\_type & {0.214} & {0.450} & {0.598} & {0.277} \\
no\_lower & {0.103} & {0.355} & {0.634} & {0.207} \\
no\_dino & {0.124} & {0.380} & {0.646} & {0.231} \\
ours & \textbf{0.090} & \textbf{0.327} & \textbf{0.671} & \textbf{0.199} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@4} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.591} & {0.796} & {0.447} & {0.457} \\
no\_type & {0.174} & {0.405} & {0.636} & {0.250} \\
no\_lower & {0.089} & {0.339} & {0.650} & {0.197} \\
no\_dino & {0.101} & {0.343} & {0.675} & {0.211} \\
ours & \textbf{0.078} & \textbf{0.308} & \textbf{0.690} & \textbf{0.187} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@5} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.588} & {0.795} & {0.449} & {0.455} \\
no\_type & {0.162} & {0.388} & {0.646} & {0.244} \\
no\_lower & {0.085} & {0.334} & {0.653} & {0.195} \\
no\_dino & {0.098} & {0.338} & {0.679} & {0.208} \\
ours & \textbf{0.076} & \textbf{0.305} & \textbf{0.692} & \textbf{0.185} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@8} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.579} & {0.787} & {0.456} & {0.452} \\
no\_type & {0.139} & {0.369} & {0.662} & {0.228} \\
no\_lower & {0.079} & {0.324} & {0.662} & {0.189} \\
no\_dino & {0.091} & {0.326} & {0.688} & {0.201} \\
ours & \textbf{0.072} & \textbf{0.295} & \textbf{0.704} & \textbf{0.178} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@10} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.578} & {0.784} & {0.459} & {0.451} \\
no\_type & {0.131} & {0.363} & {0.666} & {0.225} \\
no\_lower & {0.078} & {0.321} & {0.666} & {0.186} \\
no\_dino & {0.089} & {0.322} & {0.691} & {0.199} \\
ours & \textbf{0.070} & \textbf{0.292} & \textbf{0.706} & \textbf{0.177} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


\begin{table}
    \centering
    \resizebox{0.57\linewidth}{!}
    {
    \begin{tabular}{lcccc}
\toprule
\textbf{@16} & \textbf{DreamSim$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{SSIM$\downarrow$} & \textbf{DISTS$\downarrow$} \\
\midrule
base & {0.572} & {0.780} & {0.463} & {0.447} \\
no\_type & {0.120} & {0.350} & {0.678} & {0.216} \\
no\_lower & {0.072} & {0.311} & {0.673} & {0.180} \\
no\_dino & {0.084} & {0.315} & {0.697} & {0.194} \\
ours & \textbf{0.064} & \textbf{0.284} & \textbf{0.713} & \textbf{0.172} \\
\bottomrule
\end{tabular}
    
    }
    \caption{\textbf{Ablation Study}. We color-code results as a linear gradient between 
        \BGcolor{e0a4a4}{ w}\BGcolor{e7b2ac}{o}\BGcolor{eec0b5}{r}\BGcolor{f6cebe}{s}\BGcolor{fcdcc6}{t}\BGcolor{ffe4ca}{ }\BGcolor{fee8cc}{a}\BGcolor{feeccd}{n}\BGcolor{fdf0cf}{d}\BGcolor{f6f0cb}{ }\BGcolor{e3e6bd}{b}\BGcolor{cfdcae}{e}\BGcolor{bbd2a0}{s}\BGcolor{a8c992}{t}.
        }
    \vspace{-0.25cm}
    \label{tab:tood}
\end{table}


